Hierarchical Semi-Markov Conditional Random Fields for Recursive Sequential Data

Inspired by the hierarchical hidden Markov models (HHMM), we present the hierarchical semi-Markov conditional random field (HSCRF), a generalisation of embedded undirectedMarkov chains tomodel complex hierarchical, nestedMarkov processes. It is parameterised in a discriminative framework and has polynomial time algorithms for learning and inference. Importantly, we consider partiallysupervised learning and propose algorithms for generalised partially-supervised learning and constrained inference. We demonstrate the HSCRF in two applications: (i) recognising human activities of daily living (ADLs) from indoor surveillance cameras, and (ii) noun-phrase chunking. We show that the HSCRF is capable of learning rich hierarchical models with reasonable accuracy in both fully and partially observed data cases.

==> hcrf-apdx-partial.tex <==
%-------
Here we detail two special scenarios of the general
partial labeled data described in Section~\ref{sec:hcrf-partial}:
\begin{itemize}
\item \textbf{Case 1}: when some start and end times
	of some segments are given. This happens when we can make some
	accurate observation of the segment boundaries.
	%, i.e.	using reliable sensors in sensor-based recognition systems.
	For example, in a smart home environment, when a
	person opens the door to go out or come in, 
	the changing mode between indoor/outdoor is detected but
	we may not know exactly whether the person is going out
	or coming in. In video, topic boundary detection algorithms
	can detect the change of topics based on the change in
	the quality of images and audio, but we may
	not know the what the topics are about.
\item \textbf{Case 2}: when state variables are known
	at some time steps. This happens when we can make some accurate
	observations of the current states. For example,
	when a security officer watches a particular video of a
	monitoring system, she knows exactly what is going on at 
	that time but not how things got started and is going to end.
	Since she only has very limited time, she is only
	able to inform the system occasionally.
\end{itemize}

Although we can directly apply the general procedures outlined
in Section~\ref{sec:hcrf-partial} for these two special cases,
we provide here the more specific handling of the labeled information,
which may result in faster implementation.

%---------
\subsection{The AIO.C1 Algorithm for Case 1}
\label{sec:hcrf-AIO.C1}
%
\begin{figure}[htb]
\begin{center}
 \begin{tabular}{c}
\includegraphics[width=0.7\linewidth]{figs/observed-boundary.eps}
\end{tabular}
\end{center}
\caption{Partially labeled symmetric Markov blankets. Dashed top line
	indicates that the states are not known.}
\label{fig:observed-boundary}
\end{figure}

Case 1 is equivalent to partially observing symmetric Markov blankets 
(see Figure~\ref{fig:observed-boundary}).
Clearly, the visible joint variable $\vartheta$ defined in Section~\ref{sec:hcrf-CAIO}
is the set of all observed symmetric Markov blankets.

Recall from Section~\ref{sec:hcrf-AIO-all} that the AIO algorithm 
without constraints involves the following basic building blocks
\begin{eqnarray}
	&& \Delta^{1,s}_{1:T},\Lambda^{1,s}_{1:T} \mbox{ for } s \in S^1 \\
	&& \Delta^{d,s}_{i:j}, \Lambda^{d,s}_{i:j} \mbox{ for } d \in [2,D-1], s \in S^d, 
		1 \le i \le j \le T \\
	&& \Delta^{D,s}_{i:i},\Lambda^{D,s}_{i:i} \mbox{ for } i \in [1,T], s\in S^D \\
	&& \alpha^{1,s}_{1:j}(u),\lambda^{1,s}_{1:j}(u) \mbox{ for } s \in S^1, u \in S^{2}, j \in [1,T]\\
	&& \alpha^{d,s}_{i:j}(u), \lambda^{d,s}_{i:j}(u) 
		\mbox{ for } d \in [2,D-1], s \in S^d, u \in S^{d+1},
		1 \le i \le j \le T
\end{eqnarray}
However, with the observed symmetric Markov blankets, 
only a subset of these building blocks agrees with
the constraints. We must, therefore, identify and make use of
only those blocks that are consistent with the observations
and ignore the others. We call the new algorithm by AIO.C1, a variant
of the AIO algorithm described in Section~\ref{sec:hcrf-AIO-all}.

The new AIO.C1 algorithm proceeds in the same recursive manner as
the original AIO algorithm.  First we compute the symmetric inside
masses  and asymmetric inside masses, then use these quantities as building blocks
to compute the symmetric outside masses and asymmetric outside masses.
%------------


\subsubsection*{Computing constrained symmetric and asymmetric inside masses}
\label{sec:hcrf-AIO.C1-I-IF}
%------------

Specifically, assume that the symmetric inside mass $\Delta^{d,s}_{i:j}$
is consistent with the labels, it can be computed
from the asymmetric inside mass $\alpha^{d,s}_{i:j}(u)$ as in Equation.~\ref{I-IF}
where $u \in S^{d+1}$. However, we must check where the child state $u$
meets the constraints as follows
\begin{eqnarray}
	\label{case1-I-IF1}
	\Delta^{d,s}_{i:j} = \alpha^{d,s}_{i:j}(u)E^{d,s}_{u,j}
\end{eqnarray}
if $\tilde{x}^{d+1}_{k:j} = u$, where $k \in [i,j]$, and
\begin{eqnarray}
	\label{case1-I-IF2}
	\Delta^{d,s}_{i:j} = \sum_{u \in S^{d+1}}\alpha^{d,s}_{i:j}(u)E^{d,s}_{u,j}
\end{eqnarray}
otherwise. 

Similarly, assume the asymmetric inside mass $\alpha^{d,s}_{i:j}(u)$ is consistent for some 
$u \in S^{d+1}$, $d \in [2,D-2]$, $1 \le i \le j \le T$.
To compute $\alpha^{d,s}_{i:j}(u)$ recursively as in Equation.~\ref{IF-detail}, 
we must check whether start and end time indices of the child state $u$
are labeled, e.g. we know the start and end time of $u$ at $t$ and $j$
respectively for $t \in [i,j]$. 
\begin{itemize}
\item If we observed the start time index $t \in [i+1,j]$,  then then the asymmetric inside
	$\alpha^{d,s}_{i:j}(u)$ can be computed as
	\begin{eqnarray}
		\label{case1-IFIF1}
		\alpha^{d,s}_{i:j}(u) = \sum_{v \in S^{d+1,*}}\alpha^{d,s}_{i:t-1}(v)\hat{\Delta}^{d+1}_{t:j}(u)A^{d+1,s}_{v,u,t-1} 
	\end{eqnarray}
	where $S^{d+1,*} = S^{d+1}$ if the state $x^{d+1}_{t-1}$ is unknown,
	and $S^{d+1,*} = x^{d+1}_{t-1}$ otherwise. 
\item If $t=i$, then
	\begin{eqnarray}
		\label{case1-IFIF2}
		\alpha^{d,s}_{i:j}(u) =  \hat{\Delta}^{d+1,u}_{i:j}\pi^{d,s}_{u,i}
	\end{eqnarray}
\item If the start time $t$ for the child state $u$ is not labeled, 
	but there exists a labeled ending time index $t' \in [i,j-1]$ for some other child state
	at level $d+1$, we have
	\begin{eqnarray}
		\label{case1-IFIF3}
		\alpha^{d,s}_{i:j}(u) = \sum_{k=t'+1}^{j}\sum_{v \in S^{d+1,k}}
					\alpha^{d,s}_{i:k-1}(v)\hat{\Delta}^{d+1,u}_{k:j}A^{d+1,s}_{v,u,k-1}
	\end{eqnarray}
	where $S^{d,k} = \tilde{x}^{d+1}_{t'}$ if $k = t'+1$ and the state $x^d_{t'}$ is known, and
	$S^{d,*} = S^{d+1}$ otherwise.
\item Finally, if there are no labeled time indices within the interval $[i,j]$
	then Equation.~\ref{IF-detail} is unchanged.
\end{itemize}

For $d=1$, in Equations~\ref{case1-IFIF1},\ref{case1-IFIF2} and \ref{case1-IFIF3}, 
we must fix $i=1$. 
For $d=D-1$, the Equation~\ref{IF-special2} is rewritten as
\begin{eqnarray}
	\label{case1-IF-special2}
	\alpha^{D-1,s}_{i:j}(u)
		= \sum_{v \in S^{D,*}}\alpha^{D-1,s}_{i:j-1}(v)R^{D,u}_{j:j}A^{D,s}_{v,u,j-1}
\end{eqnarray}
where $S^{D,*} = \tilde{x}^D_{j-1}$ if we observed
the state $x^D_{j-1}$, and $S^{D,*} = S^D$ otherwise.


The recursive process is started at level $d=1$, where we
first check whether the state $s \in S^1$ is consistent to compute the
symmetric inside mass $\Delta^{1,s}_{1:T}$. For each consistent $s$, 
we compute $\Delta^{1,s}_{1:T}$ using 
Equations~\ref{case1-I-IF1} and \ref{case1-I-IF2}. The function calls
are passed downward and backward through the recursion involving
Equations~\ref{case1-IFIF1},\ref{case1-IFIF2}, and \ref{case1-IFIF3}.
The constrained partition function is computed as
\begin{eqnarray}
	Z(\vartheta) = \hat{\Delta}^{1,s}_{1:T}
\end{eqnarray}
if $s = \tilde{x}^{1}_{1:T}$, and
\begin{eqnarray}
	Z(\vartheta) = \sum_{s \in S^1}\hat{\Delta}^{1,s}_{1:T}
\end{eqnarray}
otherwise.
%------------


\subsubsection*{Estimating the constrained MAP}
\label{sec:hcrf-case2-MAP}
%------------

As we have presented in Section~\ref{sec:hcrf-MAP}, the MAP estimation is
a two-step procedure: first step is to estimate maximal joint
potential and the second step is to decode the maximal states by following
the Viterbi path. The first step is essentially a max-product version
of the AIO algorithm, where all summations are replaced by 
respective maximisations.

For the case of constrained MAP where some ending indices and states are known, 
the Viterbi path is constrained by these labels. Again, the MAP
estimation in this case is also the max-product version of the AIO.C1 algorithm.
Using the notions introduced in Section~\ref{sec:hcrf-MAP}, we rewrite
the set of equations in Section~\ref{sec:hcrf-AIO.C1-I-IF} as shown in
Table~\ref{tab:map-C1}. The last four equations in Table~\ref{tab:map-C1} correspond
to the case that there are some labeled indices and states
within the interval $[i,j]$. If this is not the case
then we can reuse the Equations~\ref{max-IF-detail},\ref{max-IF-special}
and \ref{max-IF-special2} in the unconstrained MAP estimation.

%--------------------
\begin{table}[htb]
\begin{center}
\begin{tabular}{|l|c|}
\hline
Max-product equations & Corresponding equations \\\hline\hline
$\Delta^{\max,d,s}_{i:j} = \alpha^{\max,d,s}_{i:j}(u)E^{d,s}_{u,j}$
	& Equation~\ref{case1-I-IF1} \\\hline
$\Delta^{\max,d,s}_{i:j} = \max_{u \in S^{d+1}}\alpha^{\max,d,s}_{i:j}(u)E^{d,s}_{u,j}$
	& Equation~\ref{case1-I-IF2} \\\hline
$\alpha^{\max,d,s}_{i:j}(u) = \max_{v \in S^{d+1,*}}\alpha^{\max,d}_{i:t-1}(s,v)\hat{\Delta}^{\max,d+1}_{t:j}(u)A^{d,s}_{v,u,t-1}$
	& Equation~\ref{case1-IFIF1} \\\hline
$\alpha^{\max,d,s}_{i:j}(u) =  \hat{\Delta}^{\max,d+1,u}_{i:j}\pi^{d,s}_{u,i}$
	& Equation~\ref{case1-IFIF2} \\\hline
$\alpha^{\max,d,s}_{i:j}(u) = \max_{k=t'+1}^{j}\max_{v \in S^{d+1,k}}\alpha^{\max,d,s}_{i:k-1}(v)\hat{\Delta}^{\max,d+1,u}_{k:j}A^{d+1,s}_{v,u,k-1}$
	& Equation~\ref{case1-IFIF3} \\\hline
$\alpha^{\max,D-1,s}_{i:j}(u)
		= \max_{v \in S^{D,*}}\alpha^{\max,D-1,s}_{i:j-1}(v)R^{D,u}_{j:j}A^{D,s}_{v,u,j-1}$
	& Equation~\ref{case1-IF-special2} \\\hline
\end{tabular}
\end{center}
\caption{MAP equations as max-product version of the AIO.C1.} 
\label{tab:map-C1}
\end{table}

In the second step of decoding the Viterbi path, we can reuse 
the Algorithm~\ref{alg:backtrack-map} with small modification:
in the initial step $s^* = {\arg\max}_{s \in S^1}\hat{\Delta}^{\max,1,s}_{1:T}$,
we replace $S^1$ by $S^{*,1} = \tilde{x}^1_{1:T}$ if $x^1_{1:T}$ is labeled. 


%------------
\subsubsection*{A special-special case: all ending indices are known}
%------------

If all the ending indicators are known and are hierarchically consistent, 
we can see that all the contextual cliques are activated. 
Hence, given a symmetric Markov blanket
$\Pi^{d,s}_{i:j}$, i.e. with $x^{d}_{i:j}=s$, $e^{d:D}_{i-1}=1$,
$e^{d:D}_j=1$, $e^d_{i:j-1}=0$, 
if we collapse the nodes of state $x^{d}_{i:j}$ into a single
node of state $s$, and keep all the potentials unchanged, then
we obtain a tree structured graph with small tree width.
Inference in this graph is linear in time. This 
is therefore the lower bound of the time complexity of the
AIO.C1 algorithm. 

Note that this case has been covered in the context of
Rao-Blackwellisation in Section~\ref{sec:hcrf-gibbs}, where
we have formally shown how to compute $Z(\vartheta)$ in linear time.

%---------
\subsection{The AIO.C2 Algorithm for Case 2}
\label{sec:hcrf-AIO.C2}

\begin{figure}[htb]
\begin{center}
 \begin{tabular}{c}
\includegraphics[width=0.7\linewidth]{figs/observed-state.eps}
\end{tabular}
\end{center}
\caption{For each observed state $x^d_{t_k} = s$, there must
	exists at least a symmetric Markov blanket $\Pi^{d,s}_{i:j}$
	for $t_{k-1} \le i \le t_k \le j \le t_{k+1}$.}
\label{fig:observed-state}
\end{figure}

Let $\tau^d = \{t_k\}_{k=1}^m$ be a strictly ordered set of time indices of
labeled states at level $d$, i.e. $t_{1} < t_{2} < ... < t_{m}$. 
Knowing $x^d_{t_k} = s$ would mean the state $s$ must start from $i$ and end at $j$
where $t_{k-1} \le i \le t_k \le j \le t_{k+1}$ (see Figure~\ref{fig:observed-state}).
In addition, at the same time we must ensure the hierarchical consistency, i.e.
given $e^d_t=1$ we must have $e^{d+1:D}_t=1$, and given
$e^d_t=0$, then $e^{1:d-1}_t=0$.
%-----------


\subsubsection*{Computing the constrained symmetric and asymmetric inside masses}

%-----
As in Case 1 with the AIO.C1 algorithm described in Section~\ref{sec:hcrf-AIO.C1},
ensuring the hierarchical consistency can be carried out using
the recursive function calls, starting from the 
inside at the top level $\Delta^{1,s}_{1:T}$. 
In addition, once we have correctly identified the consistent inside/asymmetric inside
variables, we can apply the same strategy
in the AIO.C1 algorithm to the AIO.C2.  What remains 
is to identify consistent inside building blocks, which
are needed to ensure the observational consistency. 


Specifically, assume that the inside $\Delta^{d,s}_{i:j}$
is consistent with the constraints, it can be computed
from the asymmetric inside $\alpha^{d,s}_{i:j}(u)$ as in Equation.~\ref{I-IF}
where $u \in S^{d+1}$. However, we must check where the child state $u$
meets the constraints as follows
\begin{eqnarray}
	\label{case2-I-IF1}
	\Delta^{d,s}_{i:j} = \alpha^{d,s}_{i:j}(u)E^{d,s}_{u,j}
\end{eqnarray}
if $t = j$ and $u = \tilde{x}^{d+1}_{j}$; and
\begin{eqnarray}
	\label{case2-I-IF2}
	\Delta^{d,s}_{i:j} = \sum_{u \in S^{d+1}}\alpha^{d,s}_{i:j}(u)E^{d,s}_{u,j}
\end{eqnarray}
otherwise. 

\begin{figure}[htb]
\begin{center}
\begin{tabular}{l}
\hline
Initialization: $\alpha^{d,s}_{i,j}(u) = 0$ \\
Set \em flag = OFF \em \\
\textbf{For} $t = j-1,j-2,...,i$ \\
\q	\textbf{If} $x^d_{t} = v$\\
\q\q		$\alpha^{d,s}_{i,j}(u) = \alpha^{d,s}_{i,j}(u) 
			+ \alpha^{d,s}_{i:t}(v)\hat{\Delta}^{d+1,u}_{t+1:j}A^{d+1,s}_{v,u,t}$\\
\q\q		Set $flag = ON$ and break the \textbf{For} loop if $v \ne u$ \\
\q	\textbf{Else} \\
\q\q		$\alpha^{d,s}_{i,j}(u) = \alpha^{d,s}_{i,j}(u) 
			+ \sum_{v\in S^{d+1}}\alpha^{d,s}_{i:t}(v)\hat{\Delta}^{d+1,u}_{t+1:j}A^{d+1,s}_{v,u,t}$\\
\q	\textbf{EndIf}\\
\textbf{If} \em flag = OFF \em \textbf{Then} $\alpha^{d,s}_{i,j}(u) = \alpha^{d,s}_{i,j}(u) + \hat{\Delta}^{d+1,u}_{i:j}E^{d,s}_{u,j}$\\
\textbf{EndFor}\\
\hline
\end{tabular}
\end{center}
\caption{Pseudo code for computing the asymmetric inside $\alpha^{d,s}_{i:j}(u)$ in Case 2
	for $d \in [1,D-2]$.}
\label{fig:forward-case2}
\end{figure}

Assume the asymmetric inside $\alpha^{d,s}_{i:j}(u)$ is consistent 
for some $u \in S^{d+1}$, $d \in [1,D-2]$, $i < j$. The pseudo code for computing
$\alpha^{d,s}_{i:j}(u)$ is presented in Figure~\ref{fig:forward-case2}.
As in the original AIO algorithm, there are two special cases: (1)
when $i=j$, then
\begin{eqnarray}
	\label{case2-IF-special}
	\alpha^{d,s}_{i:i}(u)= \hat{\Delta}^{d+1,s}_{i:i}\pi^{d,s}_{u,i}
\end{eqnarray}
and (2) for $d=D-1$, we have
\begin{eqnarray}
	\label{case2-IF-special2}
	\alpha^{D-1,s}_{i,j}(u) = \alpha^{D-1,s}_{i,j-1}(v)\hat{\Delta}^{D,u}_{j:j}A^{D,s}_{v,u,j-1}
\end{eqnarray}
if $v = \tilde{x}^{D}_{j-1}$, and
\begin{eqnarray}
	\label{case2-IF-special3}
	\alpha^{D-1,s}_{i,j}(u) = \sum_{v \in S^D}\alpha^{D-1,s}_{i,j-1}(v)\hat{\Delta}^{D,u}_{j:j}A^{D,s}_{v,u,j-1}
\end{eqnarray}
otherwise.

Similar to the AIO.C1, the AIO.C2 algorithm starts from $\Delta^{1,s}_{1:T}$ for $s \in S^1$
using Equation~\ref{case2-I-IF1} and \ref{case2-I-IF2} and
recursively passes the function calls downward and backward
using Figure~\ref{fig:forward-case2} and Equations~\ref{case2-IF-special},
\ref{case2-IF-special2} and \ref{case2-IF-special3}.
The constrained partition function is computed as
\begin{eqnarray}
	Z(\vartheta) = \hat{\Delta}^{1,s}_{1:T}
\end{eqnarray}
if $s = \tilde{x}^{1}_{1:T}$, and
\begin{eqnarray}
	Z(\vartheta) = \sum_{s \in S^1}\hat{\Delta}^{1,s}_{1:T}
\end{eqnarray}
otherwise.
%-----------

